Gravitational Lensing Simulations I : Covariance Matrices and Halo Catalogues

Gravitational lensing surveys have now become large and precise enough that the interpretation of the lensing signal has to take into account an increasing number of theoretical limitations and observational biases. Since the lensing signal is the strongest at small angular scales, only numerical simulations can reproduce faithfully the non-linear dynamics and secondary effects at play. This work is the first of a series in which all gravitational lensing corrections known so far will be implemented in the same set of simulations, using realistic mock catalogues and non-Gaussian statistics. In this first paper, we present the TCS simulation suite and compute basic statistics such as the second and third order convergence and shear correlation functions. These simple tests set the range of validity of our simulations, which are resolving most of the signals at the sub-arc minute level (or $\ell \sim 10^4$). We also compute the non-Gaussian covariance matrix of several statistical estimators, including many that are used in the Canada France Hawaii Telescope Lensing Survey (CFHTLenS). From the same realizations, we construct halo catalogues, computing a series of properties that are required by most galaxy population algorithms. These simulation products are publicly available for download.

==> halos.tex <==
\section{Halo Catalogues}
\label{sec:halo}

This section briefly describes how the halo catalogues are created, 
and presents a few of the properties that are extracted from individual objects.
We recall that our is to construct mock galaxy catalogues
on which many secondary effects will be quantified.
As mentioned before, we do not attempt to populate the haloes in this paper, since this is a challenge on its own,
and we wish to factor out this problem for now. In the future, though, one could follow \citep{2006MNRAS.371..750H}, and populate the haloes with galaxies under the conditional luminosity function of \citep{2005ApJ...627L..89C}, then assign ellipticity following the elliptical or spiral  model \citep{2000MNRAS.319..649H, 2004MNRAS.347..895H}. Alternatively, one could use the {\small GALICS} \citep{2003MNRAS.343...75H} and {\small MOMAF} \citep{2005MNRAS.360..159B} to create mock galaxy catalogues directly  our halo catalogues, following the prescription 
described in \citep{2007MNRAS.379.1507F}. Our plan is to incorporate, for the first time and in a systematic way, 
the prescriptions for intrinsic alignment, source clustering, ellipticity-shear correlation, etc. 
\citep{2007MNRAS.375....2D, 2010MNRAS.402.2127S} all at once. This is crucial in order to interpret correctly the signal from the data,
which contains all these contributions.


In this work, haloes are constructed from the matter density fields with a spherical overdensity search algorithm \citep{1996MNRAS.281..716C}. 
The first step is to assign the dark matter particles on a $2048^3$ grid with the Nearest Grid Point 
scheme \citep{1981csup.book.....H}, and identify local density  maxima. The halo finder then ranks these candidates in decreasing order of peak height, and for those which are above an inspection  threshold value, it grows a spherical volume centered on the peak, computing for each shell the integrated overdensity until it drops under the predicted critical value. The haloes that are analyzed first are then removed from the density field, in preparation for the inspection of lower mass candidates. This prevents
particles from contributing multiple times, but at the same time limits the resolution on sub-structures of the largest haloes. 
This is a mild cost for the purpose of these catalogues, which are populated with low multiplicity of galaxies,
and thus depend rather weakly on the sub-halo structures.
Finally, for each halo, we measure the mass, the centre-of-mass (CM) and peak positions, the CM velocity,
the velocity dispersion, the angular momentum in the  CM frame, and the inertia matrix $\sigma_{ij}$, 
which allows us to use population algorithms that outperform those that depend solely on the halo mass.
 Although the inertia matrix is biased by the fact that we are only searching for spherical regions,
 we still recover significant information about the shape and orientation.

In all the plots presented in this section, we present properties of the haloes that populate the full simulation box,
even though, in the final mock catalogues, we keep only those that sit inside the past light cone. 
We apply the coordinate rotation and the random shifting of the origin that was performed on the lensing slabs, such that the halo catalogues and the lenses trace the same underlying density field. 

To quantify the accuracy of the halo catalogues, we first extract the power spectrum of the distribution,
and compare the results with the measurements from dark matter particles by computing the 
halo bias, defined as $b(k) = \sqrt{P_{halo}(k) / P_{particle}(k)}$. From Fig. \ref{fig:halo_bias}, we observe that both the shape and redshift dependence agree well with the results from \cite{2011arXiv1107.4772I}. 
 We observe in Fig. \ref{fig:halo_mass} that the halo mass function is in good agreement with  \cite{1974ApJ...187..425P} and  \cite{2002MNRAS.329...61S} in the range $1 \times 10^{11} - 2 \times 10^{14} M_{\odot}$.
   Higher redshift seems to better fit Press-Schechter, while lower redshifts are better described by the Sheth-Tormen model.


%\begin{figure}
%\begin{center}
%\label{fig:halo_ps}
%\epsfig{file= graphs/HaloPower.eps,width=0.49\textwidth,height=0.49\textwidth}
%\caption{Halo power spectrum, and non-linear predictions (dotted line), for redshifts 0.961, 0.526 and 0.025 (bottom to top). 
%We include a linear bias of $1.0$, $1.14$ and $1.41$ respectively. We observe a good agreement in the linear regime, 
%with a lack of power at lower scales.}
%\end{center}
%\end{figure}

\begin{figure}
\begin{center}
\epsfig{file= graphs/fig18.eps,width=0.49\textwidth,height=0.49\textwidth}
%\epsfig{file= graphs/PS_ST_sim_0.025_3.004.eps,width=0.49\textwidth,height=0.49\textwidth}
\caption{ Halo bias, for redshifts 0.025 (bottom curve) and 0.961 (top curve). \label{fig:halo_bias}}
\end{center}
\end{figure}

   
\begin{figure}
\begin{center}
\epsfig{file= graphs/fig19.eps,width=0.49\textwidth,height=0.49\textwidth}
%\epsfig{file= graphs/PS_ST_sim_0.025_3.004.eps,width=0.49\textwidth,height=0.49\textwidth}
\caption{ {\it top: } Halo mass function, compared to predictions, for redshift 0.025, 1.071 and 3.004 (top to bottom curves). 
{\it bottom:} Ration of the mass function to the theoretical predictions of Sheth-Tormen. \label{fig:halo_mass}}
\end{center}
\end{figure}

We now present some of the relationships between the main kinematic quantities of these haloes. In Fig. \ref{fig:halo_lowZ}, \ref{fig:halo_middleZ} and \ref{fig:halo_highZ}, we show, for $z$ = 0.025, 0.961 and 3.004 respectively, and from top left to bottom right:
 the angular momentum $L$ versus the mass $m$, the halo CM velocity $v_{cm}$ versus $m$,  $L$ versus $v_{cm}$,
 then  the dispersion velocity $v_{disp}$ versus $m$, $L$ versus $v_{disp}$, and finally $\sigma$ versus $m$,
 where $\sigma$ is the angle average of the standard deviation on the centre of mass position. It is related to the
 inertia matrix via $\sigma^2 = \frac{1}{3}\sum_{i=1}^{3} \sigma^{2}_{ij}$.
 The mass is in $M_{\odot}$, the velocity is in km s$^{-1}$, the distances in $h^{-1}$Mpc, and the angular momentum in 
 $h^{-1}$Mpc km s$^{-1}$. The plots are bivariate histograms, arranged in 50x50 bins, and  the color bars are in logarithm scale for higher contrasts.
%{\bf (Should we compare to theory here?)}

\begin{figure*}
\begin{center}
\epsfig{file= graphs/fig20.eps,width=0.7\textwidth,height=0.7\textwidth}
\caption{Halo properties at $z$=0.025. {\it top, from left to right:} $L$ vs. $m$, $v_{halo}$ vs. $m$ and  $L$ vs. $v_{halo}$.
{\it bottom, from left to right:} $v_{disp}$ vs. $m$, $L$ vs. $v_{disp}$ and $\sigma$ vs. $m$. See the text for definitions of these quantities. 
The mass is in $M_{\odot}$, the velocity is in km s$^{-1}$, the distances in $h^{-1}$Mpc, and the angular momentum in $h^{-1}$ Mpc km s$^{-1}$.
The plots are bivariate histograms, where the haloes in the catalogue were bined and counted according the kinematical properties under study.
\label{fig:halo_lowZ}}
\end{center}
\end{figure*}

\begin{figure*}
\begin{center}
\epsfig{file= graphs/fig21.eps,width=0.7\textwidth,height=0.7\textwidth}
%\epsfig{file= graphs/HaloProperties_Z0.961.eps,width=0.98\textwidth,height=0.5\textwidth}
\caption{Halo properties at $z$=0.961.
The mass is in $M_{\odot}$, the velocity is in km s$^{-1}$, the distances in $h^{-1}$Mpc, and the angular momentum in $h^{-1}$Mpc km s$^{-1}$.
 \label{fig:halo_middleZ}}
\end{center}
\end{figure*}

\begin{figure*}
\begin{center}
\epsfig{file= graphs/fig22.eps,width=0.7\textwidth,height=0.7\textwidth}
\caption{Halo properties at $z$=3.004.
The mass is in $M_{\odot}$, the velocity is in km s$^{-1}$, the distances in $h^{-1}$Mpc, and the angular momentum in $h^{-1}$Mpc km s$^{-1}$.
 \label{fig:halo_highZ}}
\end{center}
\end{figure*}



